Estimating Stellar Atmospheric Parameters by Automated Methods Using SSLs

Libraries of stellar spectra, such as ELODIE (Prugniel & Soubiran 2001), CFLIB (Valdes et al. 2004), or MILES (S\'anchez-Bl\'azquez et al. 2006), are used for a variety of applications, and especially in modelling stellar populations (e. g. Le Borgne et al. (2004)). In that context, apart from the completeness and quality of these spectral databases (Singh et al. 2006), the accurate calibration of stellar atmospheric parameters, temperature (Teff), surface gravity (log g), and metallicity ([Fe/H]), is known to be critical (Prugniel et al. 2007; Percival & Salaris 2009). We discuss the technique of determining stellar atmospheric parameters accurately by `full spectrum fitting'.

==> table12.tex <==
NGC288    & 1    & $  -1.35 \pm    0.05$ &    -   & $  -0.03$ \\
NGC1904   & 3    & $  -1.69 \pm    0.05$ &   0.04 & $  -0.09$ \\
NGC2420   & 1    & $  -0.28 \pm    0.03$ &    -   & $   0.03$ \\
NGC2682   & 1    & $  -0.07 \pm    0.03$ &    -   & $  -0.07$ \\
NGC5272   & 3    & $  -1.53 \pm    0.06$ &   0.05 & $  -0.03$ \\
NGC5904   & 2    & $  -1.37 \pm    0.04$ &   0.06 & $  -0.07$ \\
NGC6205   & 1    & $  -1.42 \pm    0.03$ &    -   & $   0.11$ \\
NGC6341   & 2    & $  -2.41 \pm    0.05$ &   0.12 & $  -0.10$ \\
IC 4725   & 1    & $  -0.02 \pm    0.03$ &    -   & $  -0.05$ \\
NGC6791   & 3    & $   0.32 \pm    0.03$ &   0.09 & $  -0.10$ \\
NGC6838   & 17   & $  -0.86 \pm    0.08$ &   0.07 & $  -0.08$ \\
NGC7789   & 11   & $  -0.04 \pm    0.03$ &   0.05 & $  -0.05$ \\



